ENFrame: A Platform for Processing Probabilistic Data

This paper introduces ENFrame, a unified data processing platform for querying and mining probabilistic data. Using ENFrame, users can write programs in a fragment of Python with constructs such as bounded-range loops, list comprehension, aggregate operations on lists, and calls to external database engines. The program is then interpreted probabilistically by ENFrame. The realisation of ENFrame required novel contributions along several directions. We propose an event language that is expressive enough to succinctly encode arbitrary correlations, trace the computation of user programs, and allow for computation of discrete probability distributions of program variables. We exemplify ENFrame on three clustering algorithms: k-means, k-medoids, and Markov Clustering. We introduce sequential and distributed algorithms for computing the probability of interconnected events exactly or approximately with error guarantees. Experiments with k-medoids clustering of sensor readings from energy networks show orders-of-magnitude improvements of exact clustering using ENFrame over na\"ive clustering in each possible world, of approximate over exact, and of distributed over sequential algorithms.

==> settings.tex <==
\usepackage{color}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage[normalem]{ulem}
\usepackage{verbatim}
\usepackage{enumitem}

\RequirePackage{xspace,amsmath,amssymb,upgreek,varioref}


\makeatletter
\newif\if@restonecol
\makeatother
\let\algorithm\relax
\let\endalgorithm\relax
\usepackage[ruled,vlined]{algorithm2e}
% \SetAlCapSkip{0.5em}
% \SetAlCapNameSty{textbf}
\SetAlCapHSkip{0cm}
\SetAlgoSkip{}
\setlength{\algomargin}{0em}
\SetKwComment{Comment}{$\rhd$~}{}
\SetKwBlock{Begin}{}{}
\SetKw{Output}{output}
\SetKw{Choose}{choose}
\SetFuncSty{textsc} 
\SetCommentSty{scriptsize}
\SetDataSty{textsc}

%\usepackage{tikz}
% \usetikzlibrary{arrows} %,shapes,automata}
% \usetikzlibrary{decorations.pathreplacing,calc,patterns,backgrounds}
% \definecolor{orange}{rgb}{1,0.5,0}
% \definecolor{myblue}{rgb}{0.2,0.35,0.8}
% 
% \usepackage{pgfplots}
% \pgfplotsset{compat=1.5,log origin=infty, every axis title shift=1pt, unbounded coords=jump}

% \usetikzlibrary{external}
%\tikzexternalize 

\newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \newtheorem{corollary}{Corollary}

% No italics for the following environments:
\theoremstyle{definition}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition} 
% \newdefinition{remark}{Remark} 

\newcommand{\dd}{\partial}
\newcommand{\dist}{\ensuremath{\text{dist}}}
\newcommand{\cfS}{\ensuremath{\mathcal{S}}}
\newcommand{\cfI}{\ensuremath{\mathcal{I}}}
\newcommand{\cfF}{\ensuremath{\mathcal{F}}}
\newcommand{\cfM}{\ensuremath{\mathcal{M}}}
\newcommand{\cfL}{\ensuremath{\mathcal{L}}}
\newcommand{\cfC}{\ensuremath{\mathcal{C}}}
\newcommand{\cfB}{\ensuremath{\mathcal{B}}}
\newcommand{\cfV}{\ensuremath{\mathcal{V}}}
\newcommand{\cfO}{\ensuremath{\mathcal{O}}}
\newcommand{\cfD}{\ensuremath{\mathcal{D}}}
\newcommand{\cfIQ}{\ensuremath{\mathcal{IQ}}}
\newcommand{\cfEL}{\ensuremath{\mathcal{EL}}}
\newcommand{\cfUL}{\ensuremath{\mathcal{UL}}}

\newcommand{\bbR}{\ensuremath{\mathbb{R}}}

\newcommand{\bfu}{\ensuremath{\mathbf{u}}}
\newcommand{\bfx}{\ensuremath{\mathbf{x}}}
\newcommand{\bfy}{\ensuremath{\mathbf{y}}}
\newcommand{\bfO}{\ensuremath{\mathbf{O}}}
\newcommand{\bfX}{\ensuremath{\mathbf{X}}}

\newcommand{\rpunto}{\tag*{\hspace{-1em}$\Box$}} % Punto when last line is \[\]
\newcommand{\punto}{\hfill\ $\Box$}

\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\rob}[1]{\textcolor{blue}{ROB: #1}}
\newcommand{\dan}[1]{\textcolor{blue}{DAN: #1}}

\newcommand{\nop}[1]{}
% \newcommand{\conditionalPicture}[1]{}
\newcommand{\conditionalPicture}[1]{#1}
\newcommand{\tuple}[1]{{\langle#1\rangle}}
\def\lBrack{\lbrack\!\lbrack}
\def\rBrack{\rbrack\!\rbrack}
\newcommand{\Bracks}[1]{\lBrack#1\rBrack}

\newcommand{\cpar}[1]{ {\smallskip\noindent\bf #1} }

\renewcommand{\vec}[1]{\mathbf{#1}}

\newcommand{\kmedoids}{$k$-medoids\xspace}
\newcommand{\kmeans}{$k$-means\xspace}

\hyphenation{da-ta-base da-ta-bases ap-prox-i-ma-tion up-date ar-bi-trar-ily EPSRC}

\renewcommand{\baselinestretch}{0.965}
